8DNA: 8D Neural Asset Light Transport by Distribution Learning

High-fidelity 3D assets exhibit intriguing global illumination effects like subsurface scattering, glossy interreflections, and fine-scale fiber scatterings, which often involve long scattering paths that are expensive to simulate. We introduce 8D neural assets (8DNA) to pre-bake these light transport effects into neural representations. Unlike prior methods that assume far-field lighting and precompute light transport into 6D functions, 8DNA learns the full 8D light transport, enabling accurate rendering under near-field illumination. Our training leverages a distribution-learning formulation that learns light transport from forward path-traced samples, which produces less optimization variance with lower training budget than the prior regression-based approaches. Experiments show our 8DNA rendering closely matches path-traced results under various scene configurations, yet it achieves improved variance reduction and fast inference speeds on challenging assets.

==> equations/2-gtf.tex <==
\begin{equation}
\begin{split}
    \fnear(\xxo,\omegao,\omegai)&=
    \int \fnear(\xxo,\omegao,\bo)\delta_{\omegai}(\bo)\mathrm{d}\bo
    \\
    &=\capl_{pt}(\xxo,\omegao,\delta_{\omegai}).
\end{split}
\label{eq:2-gtf}
\end{equation}

==> equations/2-vlte.tex <==
\begin{equation}
\begin{split}
\capl_o&(\xxo,\omegao)=\int_{0}^{+\infty}\!\!\!\!\!\!\mathbf{T}(\xxo,t)
\Big( \bm{\sigma}_a(\xxo(t)) \capl_i(\xxo(t),\omegao)\\
&+\bm{\sigma}_s(\xxo(t))\!\!\int \!\!\capf(\xxo(t),\omegao,\omegai) \capl_o(\xxo(t),-\omegai)\Big)
    \mathrm{d}t\mathrm{d}\omegai;\\
\end{split}
\label{eq:2-vlte}
\end{equation}

==> equations/3-albedo.tex <==
\begin{equation}
    \bm{\alpha}(\xxo,\omegao)=\!\!\mathop{\mathbb{E}}_{\xxi,\omegai,\bm{\beta}_i\sim \text{path sampling}}
    \!\!\left[
    \bm{\beta}_i
    \right].
\label{eq:3-albedo}
\end{equation}

==> equations/3-autoregressive.tex <==
\begin{equation}
%\begin{split}
\mathbf{p}_{\bm{\theta}}(
\mathbf{s}|\xxo,\omegao
)
=\prod_{j=1}^{4}
\mathbf{p}_{\bm{\theta}}(
\mathbf{s}^j| \mathbf{s}^{k<j}, \xxo,\omegao
);
%\mathbf{p}_{\bm{\theta}}(s_1|\xxo,\omegao)
%\mathbf{p}_{\bm{\theta}}(s_2|s_1,\xxo,\omegao)\\
%\times\;\mathbf{p}_{\bm{\theta}}(s_3|s_2,s_1,\xxo,\omegao)
%\mathbf{p}_{\bm{\theta}}(s_4|s_3,s_2,s_1,\xxo,\omegao);
%\end{split}
\label{eq:3-autoregressive}
\end{equation}

==> equations/3-emitter-sampling.tex <==
\begin{equation}
\capl = \capl +
\bm{\beta}w_e
\frac{
\capl_e(\mathbf{u}_i,\omegai)
\capf_{\bm{\theta}}(\mathbf{u}_i,\omegai)
}{\mathbf{p}_{\bm{\theta}}^c(\mathbf{u}_i)p_e(\omegai|\mathbf{u}_i)},
w_e = 
\tfrac{p_e(\omegai|\mathbf{u}_i)^2}
{
\mathbf{p}_{\bm{\theta}}^c(\omegai|\mathbf{u}_i)^2
+p_e(\omegai|\mathbf{u}_i)^2
}.
\label{eq:3-emitter-sampling}
\end{equation}

==> equations/3-nll.tex <==
\begin{align}
-\iint \mathbf{p}\log\mathbf{p}_\theta
\mathrm{d}\xxi\mathrm{d}\omegai
=-\frac{1}{\bm{\alpha}}\iint \capf\log\mathbf{p}_\theta
\mathrm{d}\xxi\mathrm{d}\omegai.
\tag*{}
\end{align}

==> equations/3-path-sampling.tex <==
\begin{equation}
\begin{split}
\mathop{\mathbb{E}}_{\omegai\sim\mathbf{p}_{\bm{\theta}}^c(\omegai|\xxi,\cdot)}
\left[
w_\text{path}
\frac{
\capl_e(\mathbf{u}_i,\omegai)\capf_{\theta}(\mathbf{u}_i,\omegai,\xxo,\omegai)
}{
\mathbf{p}_{\bm{\theta}}^c(\mathbf{u}_i|\xxo,\omegao)
\mathbf{p}_{\bm{\theta}}^c(\omegai|\mathbf{u}_i,\xxo,\omegao)
}
\right]\\
w_\text{path} = 
\tfrac{\mathbf{p}_{\bm{\theta}}^c(\omegai|\mathbf{u}_i,\xxo,\omegao)^2}
{
\mathbf{p}_{\bm{\theta}}^c(\omegai|\mathbf{u}_i,\xxo,\omegao)^2
+p_\text{emit}(\omegai|\mathbf{u}_i)^2
}.
\end{split}
\end{equation}

==> equations/3-rqs-MLP.tex <==
\begin{equation}
\mathbf{g}_j=\text{MLP}_j(
\mathbf{s}^{k<j},\xxo,\omegao,
\bm{\theta}),
\label{eq:3-rqs-MLP}
\end{equation}

==> equations/6-direct-indirect-estimator.tex <==
\begin{equation}
\mathbf{I}=
\begin{cases}
    \frac{1}{m}\frac{V(\xxo,\bo'_i)\mathbf{f}(\xxo,\omegao,\omegai')}{p_\capf(\bo'_i|\xxo)}\capl_i(\xxo,\omegai')&
    \text{with probability }m\\
    \frac{1}{1-m}\frac{\capf_{\bm{\theta}}(\xxo,\omegao,\xxi,\omegai)}{\mathbf{p}^c_{\bm{\theta}}(\xxi,\omegai|\xxo,\omegao)}\capl_i(\xxi,\omegai) & \text{otherwise}
\end{cases}
,
\end{equation}

==> equations/6-direct-indirect.tex <==
\begin{gather}
\mathop{\mathbb{E}}_{\xxi,\omegai,\omegai',m}\left[
\mathbf{I}
\right]=
\mathop{\mathbb{E}}_{\xxi,\omegai,\omegai'}\left[
m\frac{1}{m}\frac{V\mathbf{f}}{p_\mathbf{f}}\capl_i
+(1-m)\frac{1}{1-m}\frac{\capf_{\bm{\theta}}}{\mathbf{p}^c_{\bm{\theta}}}\capl_i\right]
\tag*{}\\
=\iiint\!\!\!
\mathbf{p}^c_{\bm{\theta}}(\xxi,\omegai)
\left(p_\mathbf{f}(\omegai')
\frac{V(\bo'_i)\mathbf{f}(\omegai')}{p_\mathbf{f}(\bo'_i)}\capl_i(\xxo,\omegai')
\mathrm{d}\bo'_i\right)\mathrm{d}\xxi\mathrm{d}\omegai
\tag*{}\\
+
\iiint\!\!\!
p_\mathbf{f}(\omegai')
\left(
\mathbf{p}^c_{\bm{\theta}}(\xxi,\omegai)
\frac{\capf_{\bm{\theta}}(\xxi,\omegai)}{\mathbf{p}^c_{\bm{\theta}}(\xxi,\omegai)}\capl_i(\xxi,\omegai)
\mathrm{d}\xxi\mathrm{d}\omegai\right)\mathrm{d}\bo'_i
\tag*{}\\
=\int\!\!\!
V(\bo'_i)\mathbf{f}(\omegai')\capl_i(\xxo,\omegai')
\mathrm{d}\bo'_i
+\!\!\iint\!\!\!
\capf_{\bm{\theta}}(\xxi,\omegai)\capl_i(\xxi,\omegai)
\mathrm{d}\xxi\mathrm{d}\omegai.
\tag*{}
\end{gather}

==> tables/2-notation.tex <==
\begin{table}[t]
    \centering
    %\setlength\tabcolsep{3 pt}
    \caption{\textbf{Notations.}}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{ll}
        \toprule
        Symbol & Definition \\
        \midrule
        $\mathbf{v}^j$ & $j$th component of vector $\mathbf{v}$\\
        %$\delta_{\bx'}(\bx)$ & Dirac-delta function $\delta(\bx-\bx')$\\
        $\bx,\bo$ & position $\in$ 2D surface $\surface$, direction $\in$ sphere $\sphere$\\
        $\xxi,\omegai$ & incident (light) position, direction\\
        $\xxo,\omegao$ & outgoing (camera) position direction\\
        $\mathbf{u}_i$ & incident location $\in$ the asset bounding box $\mathcal{B}$\\
        %$\mathbf{n}_{\bx}$ & surface normal at $\bx$\\
        $\capl_i(\bx,\bo)$ & incident radiance from the rest of the scene\\
        $\capl_o(\bx,\bo;\mathbf{L}_i)$ & outgoing radiance under incident light $\mathbf{L}_i$\\
        %$L_i(\bx,\bo),L_o(\bx,\bo)$ & incident, outgoing radiance\\
        %$\capf(\bx,\omegao,\omegai)$ & cosine-weighted BSDF/phase function\\
        \bottomrule
    \end{tabular}
    }
    \label{tab:2-notation}
\end{table}
